Versatile Physical Properties of a Novel Two-Dimensional Materials Composed of Group IV-V Elements

Owing to the fascinating physical characteristics of two-dimensional (2D) materials and their heterostructure, much effort has been devoted to exploring their basic physical properties as well as discovering other novel 2D materials. Herein, based on first-principles calculations, we propose novel 2D material groups with the form A$_2$B$_2$, composed of group IV (A = C, Si, Ge, or Sn) and V (B = N, P, As, Sb, or Bi) elements; the group forms two stable phases with the $P\bar{6}m2$ ($\mathcal{M}$ phase) and $P\bar{3}m1$ ($\mathcal{I}$ phase) crystal symmetries. We found that a total of 40 different freestanding A$_2$B$_2$ compounds were dynamically stable and displayed versatile physical properties, such as insulating, semiconducting, or metallic properties, depending on their elemental compositions. Our calculation results further revealed that the newly proposed 2D materials expressed high electrical and thermal transport properties. Additionally, some of the compounds that contained heavy elements exhibited non-trivial topological properties due to strong spin-orbit interactions.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
